Enhancing Energy System Models Using Better Load Forecasts

Energy system models require a large amount of technical and economic data, the quality of which significantly influences the reliability of the results. Some of the variables on the important data source ENTSO-E transparency platform, such as transmission system operators' day-ahead load forecasts, are known to be biased. These biases and high errors affect the quality of energy system models. We propose a simple time series model that does not require any input variables other than the load forecast history to significantly improve the transmission system operators' load forecast data on the ENTSO-E transparency platform in real-time, i.e., we successively improve each incoming data point. We further present an energy system model developed specifically for the short-term day-ahead market. We show that the improved load data as inputs reduce pricing errors of the model, with strong reductions particularly in times when prices are high and the market is tight.

==> Tables/T_MSE_priceestimator_allyears.tex <==
\begin{table}[H]
	\begin{center}
	\small
		\begin{tabular}{|l||r|r|r|r|r|r|r|r|}
			\hline
			\multicolumn{1}{|c||}{ } &
			\multicolumn{2}{c|}{all years} &
			\multicolumn{2}{c|}{2017} &
			\multicolumn{2}{c|}{2018} &
			\multicolumn{2}{c|}{2019} \\
			\hline
			 & Impr. & Orig & Impr & Orig & Impr & Orig & Impr & Orig  \\
			\hline
			[1] MSE  & 89.15 & 90.73 & 133.13 & 135.29 & 72.47 & 73.22 & 61.84 & 63.70 \\
			\hline
			[2] RMSE  & 9.44 & 9.53 & 11.54 & 11.63 & 8.51 & 8.56 & 7.86 & 7.98 \\
			\hline
			[3] MAE & 5.94 & 5.96 & 6.75 & 6.80 & 5.98 & 6.04 & 5.09 & 5.28 \\
			\hline
			Reduction [1] & 1.75\% & & 1.62\% & & 1.04\% &  & 3.01\% & \\
			\hline
			Reduction [2] & 0.88\% &  & 0.81\% &  & 0.52\% & & 1.49\% &  \\
			\hline
			Reduction [3] & 0.42\% &  & 0.85\% & & 1.02\% & & 3.65\% &  \\
			\hline
			
		\end{tabular}
		\bigskip
		\caption{Error measures for the price estimator of the em.power dispatch model comparing the improved load forecasts (Impr.) by original load forecasts (Orig), given in [$MWh^2$] for MSE, in [$MWh$] for RMSE and MAE.}
		
		\label{table_errormeasures_price_allyears}
	\end{center}
\end{table}

==> Tables/T_load_desc_hourly.tex <==
\begin{table}[H]
	\begin{center}
	\small
		\begin{tabular}{|l||r|r|r|r|r|r|r|}
			\hline
			Hour	&	Mean	& Median & 	Minimum	&	Maximum	&	5\%-quantile	&	95\%-quantile	&	Std.	\\
			\hline
            1	&	699.64	&	742.75	&	-5710.00	&	6594.75	&	-2270.28	&	3509.15	&	1713.19	\\
            2	&	652.07	&	696.75	&	-6302.25	&	6701.50	&	-2290.58	&	3460.69	&	1711.79	\\
            3	&	646.41	&	657.75	&	-6558.25	&	6882.75	&	-2246.04	&	3535.18	&	1739.51	\\
            4	&	690.28	&	687.50	&	-8539.00	&	6888.25	&	-2269.38	&	3635.30	&	1760.22	\\
            5	&	855.45	&	852.75	&	-15353.75	&	7617.25	&	-2298.63	&	3959.94	&	1991.04	\\
            6	&	943.53	&	1032.50	&	-17543.50	&	9113.00	&	-2658.48	&	4335.81	&	2295.79	\\
            7	&	946.49	&	1075.75	&	-20358.00	&	11469.00	&	-2896.14	&	4688.48	&	2515.40	\\
            8	&	912.14	&	1011.00	&	-19681.75	&	11152.25	&	-2795.23	&	4529.93	&	2461.27	\\
            9	&	908.80	&	959.00	&	-16540.25	&	11658.25	&	-2692.56	&	4594.01	&	2387.68	\\
            10	&	902.67	&	900.00	&	-15234.63	&	12930.75	&	-2836.34	&	4707.63	&	2417.03	\\
            11	&	916.34	&	926.75	&	-14149.88	&	10484.25	&	-2791.68	&	4646.26	&	2401.02	\\
            12	&	923.30	&	951.00	&	-14261.88	&	10471.25	&	-2818.44	&	4782.05	&	2414.55	\\
            13	&	907.81	&	982.00	&	-15839.88	&	9777.25	&	-2980.00	&	4740.98	&	2446.60	\\
            14	&	785.04	&	882.75	&	-15116.63	&	9306.75	&	-2963.74	&	4549.70	&	2412.79	\\
            15	&	718.73	&	807.50	&	-15220.38	&	9510.50	&	-2933.24	&	4477.88	&	2396.13	\\
            16	&	900.33	&	895.50	&	-14434.38	&	9520.25	&	-2777.48	&	4756.91	&	2323.86	\\
            17	&	1080.73	&	1051.50	&	-13068.00	&	9951.25	&	-2526.88	&	4832.60	&	2285.24	\\
            18	&	1172.53	&	1128.00	&	-12133.38	&	10094.50	&	-2110.33	&	4819.08	&	2140.34	\\
            19	&	1180.48	&	1161.25	&	-11652.75	&	9409.75	&	-1985.76	&	4610.81	&	2078.72	\\
            20	&	1061.99	&	1071.00	&	-9940.75	&	8430.50	&	-1956.98	&	4248.70	&	1978.27	\\
            21	&	875.01	&	909.25	&	-8443.13	&	7422.00	&	-2121.79	&	3943.60	&	1888.30	\\
            22	&	877.85	&	872.75	&	-6668.50	&	6932.25	&	-2032.00	&	3853.51	&	1821.24	\\
            23	&	863.47	&	806.00	&	-5642.38	&	6947.25	&	-1928.34	&	3706.63	&	1726.26	\\
            24	&	729.88	&	763.25	&	-5607.88	&	7011.50	&	-2262.01	&	3560.98	&	1701.36	\\


            
			\hline
			
		\end{tabular}
		\bigskip
		\caption{Hourly averaged descriptive statistics of TSO load forecast errors for the years 2016 - 2019.}
		
		\label{table_descriptives_load_allyears_hourly}
	\end{center}
\end{table}

==> Tables/T_load_desc_weekday.tex <==
\begin{table}[H]
	\begin{center}
	\small
		\begin{tabular}{|l||r|r|r|r|r|r|r|}
			\hline
				&	Mean	&	Median	&	Minimum	&	Maximum	&	5\%-quantile	&	95\%-quantile	&	Std.	\\
			\hline
                Mon.	&	1517.71	&	1436.63	&	-6277.00	&	12930.75	&	-1895.75	&	5111.45	&	2159.26	\\
                Tue.	&	1685.17	&	1581.50	&	-4867.25	&	11469.00	&	-1473.05	&	5126.95	&	1984.32	\\
                Wed.	&	1601.81	&	1516.00	&	-7868.50	&	9053.75	&	-1242.65	&	4667.90	&	1874.89	\\
                Thu.	&	1361.43	&	1365.25	&	-17543.50	&	9520.25	&	-1372.88	&	4330.47	&	1896.08	\\
                Fri.	&	944.31	&	990.75	&	-10596.88	&	9772.25	&	-2060.85	&	3911.48	&	1892.38	\\
                Sat.	&	-102.26	&	-43.63	&	-7661.75	&	7809.00	&	-2967.80	&	2380.13	&	1696.76	\\
                Sun.	&	-378.19	&	-340.13	&	-7752.50	&	7522.00	&	-3378.53	&	2458.15	&	1859.72	\\


            
			\hline
			
		\end{tabular}
		\bigskip
		\caption{Weekday wise descriptive statistics of TSO load forecast errors for the years 2016 - 2019.}
		
		\label{table_descriptives_load_allyears_weekday}
	\end{center}
\end{table}

==> Tables/T_load_descriptives.tex <==
\begin{table}[htb]
	\begin{center}
	\small
		\begin{tabular}{|l||r|r|r|r|r|r|r|r|}
			\hline
				    &	all	&	2016	&	2017	&	2018	&	2019	\\
            \hline
            Mean	&	881.29	&	1,555.38	&	446.50	&	298.60	&	1,222.84	\\
            Median	&	892.75	&	1,468.00	&	479.50	&	395.63	&	1,195.75	\\
            Minimum	&	-20,358.00	&	-7,752.50	&	-7,868.50	&	-20,358.00	&	-7,415.00	\\
            Maximum	&	12,930.75	&	12,930.75	&	8,392.50	&	9,045.25	&	9,635.25	\\
            5\%-quantile	&	-2,477.50	&	-1,684.03	&	-2,413.75	&	-3,180.63	&	-2,266.13	\\
            95\%-quantile	&	4,294.40	&	4,894.20	&	3,099.38	&	3,644.75	&	4,811.38	\\
            Std.	&	2,149.75	&	2,079.19	&	1,746.54	&	2,341.68	&	2,128.55	\\
            LB hypothesis	&	1.00	&	1.00	&	1.00	&	1.00	&	1.00	\\
			\hline
			
		\end{tabular}
		\bigskip
		\caption{Descriptive statistics of TSO load forecast errors for the years 2016 to 2019. Except LB hypothesis, all variables are given in [$MWh$].}
		
		\label{table_descriptives_load_allyears}
	\end{center}
\end{table}

==> Tables/T_loadimprovementMSEMAEyearly.tex <==
\begin{table}[H]
	\begin{center}
	\small
		\begin{tabular}{|l|l||r|r|r|r|r|r|r|}
			\hline
				&	year	&	all	&	2017	&	2018	&	2019	\\
			\hline
			Mean	&	TSO	&	655.98	&	446.50	&	298.60	&	1,222.84	\\
            	&	Impr.	&	-98.89	&	-229.06	&	-36.32	&	-31.29	\\
            \hline
            Std.	&	TSO	&	2,125.72	&	1,746.54	&	2,341.68	&	2,128.55	\\
            	&	Impr.	&	1,743.89	&	1,465.74	&	2,043.67	&	1,665.56	\\
            \hline
            	&	TSO	&	4,948,990.80	&	3,249,416.14	&	5,572,010.71	&	6,025,545.56	\\
            MSE	&	Impr.	&	3,050,928.19	&	2,200,617.23	&	4,177,415.90	&	2,774,751.43	\\
            	&	\% Improvement	&	38.35	&	32.28	&	25.03	&	53.95	\\
            \hline
            	&	TSO	&	2,224.63	&	1,802.61	&	2,360.51	&	2,454.70	\\
            RMSE	&	Impr.	&	1,746.69	&	1,483.45	&	2,043.87	&	1,665.76	\\
            	&	\% Improvement	&	21.48	&	17.71	&	13.41	&	32.14	\\
            \hline
            	&	TSO	&	1,691.37	&	1,396.45	&	1,726.67	&	1,951.00	\\
            MAE	&	Impr.	&	1,253.95	&	1,106.12	&	1,372.55	&	1,283.17	\\
            	&	\% Improvement 	&	25.86	&	20.79	&	20.51	&	34.23	\\
			\hline
			
		\end{tabular}
		\bigskip
		\caption{Means, standard deviations (Std.) and error measures (MSE, RMSE, MAE) for the original TSO day-ahead load forecast (TSO) and the improved day-ahead load forecast (Impr.). MSE is given in [$MWh^2$], all other variables in [$MWh$].}
		
		\label{table_errormeasures_load_allyears}
	\end{center}
\end{table}


==> Tables/T_loadimprovementMSEMAEyearly_3MRW.tex <==
\begin{table}[h]
	\begin{center}
	\small
		\begin{tabular}{|l|l||r|r|r|r|r|r|r|}
			\hline
				&	all	&	2017	&	2018	&	2019	\\
			\hline
            MSE	&	4948990.80	&	2272350.07	&	4575637.58	&	3133176.51	\\
            RMSE	&	2224.63	&	1507.43	&	2139.07	&	1770.08	\\
            MAE	&	1691.37	&	1132.86	&	1462.48	&	1377.82	\\

			\hline
			
		\end{tabular}
		\bigskip
		\caption{Error measures (MSE, RMSE, MAE) for the the improved day ahead-load forecast with a rolling window length of three month. MSE is given in [$MWh^2$], RMSE and MAE in [$MWh$].}
		
		\label{table_errormeasures_3mRW_allyears}
	\end{center}
\end{table}

==> Tables/T_loadimprovementMSEMAEyearly_6MRW.tex <==
\begin{table}[h]
	\begin{center}
	\small
		\begin{tabular}{|l|l||r|r|r|r|r|r|r|}
			\hline
				&	all	&	2017	&	2018	&	2019	\\
			\hline
            MSE	&	4016010.14	&	4896546.88	&	4355814.17	&	2795669.38	\\
            RMSE	&	2004.00	&	2212.81	&	2087.06	&	1672.03	\\
            MAE	&	1304.12	&	1200.16	&	1411.57	&	1300.63	\\


			\hline
			
		\end{tabular}
		\bigskip
		\caption{Error measures (MSE, RMSE, MAE) for the the improved day-ahead load forecast with a rolling window length of six month. MSE is given in [$MWh^2$], RMSE and MAE in [$MWh$].}
		
		\label{table_errormeasures_3mRW_allyears}
	\end{center}
\end{table}

==> Tables/T_loadimprovement_weekdaywise.tex <==
\begin{table}[H]
	\begin{center}
	\small
		\begin{tabular}{|l||r|r|r|r|r|r|}
			\hline
			\multicolumn{1}{|c||}{} &
			\multicolumn{3}{c|}{MSE} &
			\multicolumn{3}{c|}{MAE} \\
				    &	TSO	&	Impr.	&	\% Improvement	&	TSO	&	Impr.	&	\% Improvement\\
			\hline
            Monday	&	5775547.56	&	2936124.57	&	49.16	&	1898.94	&	1285.17	&	32.32	\\
            Tuesday	&	5402385.55	&	2550582.51	&	52.79	&	1840.46	&	1231.75	&	33.07	\\
            Wednesday	&	5257605.88	&	2647820.42	&	49.64	&	1794.89	&	1234.17	&	31.24	\\
            Thursday	&	5139608.31	&	3108376.72	&	39.52	&	1716.29	&	1221.29	&	28.84	\\
            Friday	&	4465707.19	&	2698216.19	&	39.58	&	1637.75	&	1229.77	&	24.91	\\
            Saturday	&	2905826.70	&	2344292.87	&	19.32	&	1329.09	&	1142.35	&	14.05	\\
            Sunday	&	3503699.47	&	2304541.42	&	34.23	&	1478.88	&	1160.33	&	21.54	\\
			\hline
			
		\end{tabular}
		\bigskip
		\caption{Weekday wise error measures for the original TSO day-ahead load forecast and the improved day-ahead load forecast. MSE is given in [$MWh^2$], MAE in [$MWh$], Improvement in [\%].}
		
		\label{table_errormeasures_load_weekdaywise}
	\end{center}
\end{table}
